Motivic Integration and Logarithmic Geometry

In this thesis, we use logarithmic methods to study motivic objects. Let R be a complete discrete valuation ring with perfect residue field k, and denote by K its fraction field. We give in chapter 2 a new construction of the motivic Serre invariant of a smooth K-variety and extend it additively to arbitrary K-varieties. The main advantage of this construction is to rely only on resolution of singularities and not on a characteristic zero assumption, as did previous results. As an application, we give a conditional positive answer to Serre's question on the existence of rational fixed points of a G-action on the affine space, for G a finite l-group. We end the chapter by showing how the logarithmic point of view that we use in our construction leads to a new understanding of the motivic nearby cycles with support of Guibert, Loeser and Merle as a motivic volume. In chapter 4 we use the theory of logarithmic geometry to derive a new formula for the motivic zeta function via the volume Poincar\'e series. More precisely, we show how to compute the volume Poincar\'e series associated to a generically smooth log smooth R-scheme in terms of its log geometry, more specifically in terms of its associated fan in the sense of Kato. This formula yields a much smaller set of candidate poles for the motivic zeta function and seems especially well suited to tackle the monodromy conjecture of Halle and Nicaise for Calabi-Yau K-varieties, for which log smooth models appear naturally through the Gross-Siebert programme on mirror symmetry. We end the chapter by showing how this formula sheds new light on previous results regarding the motivic zeta function of a polynomial nondegenerate with respect to its Newton polyhedron, and of a polynomial in two variables.

==> chapters/abstract/Makefile <==
# Autogenerated Makefile, Wed Dec  3 15:26:40 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: abstract.pdf
abstract.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstract/$@ )

.PHONY: bare abstract_bare.pdf
bare: abstract_bare.pdf
abstract_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstract/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/abstract/abstract.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard abstract*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) abstract.pdf abstract_bare.pdf

s:
	@echo gvim abstract.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/abstract/abstract.tex <==
\chapter{Abstract} \label{ch:abstract}


In this thesis, we use logarithmic methods to study motivic objects.
Let $R$ be a complete discrete valuation ring with perfect residue field~$k$, and denote by $K$ its fraction field.
We give in chapter~\ref{ch:serre} a new construction of the motivic Serre invariant of a smooth $K$-variety and extend it additively to arbitrary $K$-varieties.
The main advantage of this construction is to rely only on resolution of singularities and not on a characteristic zero assumption, as did previous results.
As an application, we give a conditional positive answer to Serre's question on the existence of rational fixed points of a $G$-action on the affine space, for $G$ a finite $\ell$-group.
We end the chapter by showing how the logarithmic point of view that we use in our construction leads to a new understanding of the motivic nearby cycles with support of Guibert, Loeser and Merle as a motivic volume.

In chapter~\ref{ch:log} we use the theory of logarithmic geometry to derive a new formula for the motivic zeta function via the volume Poincaré series.
More precisely, we show how to compute the volume Poincaré series associated to a generically smooth log smooth $R$-scheme in terms of its log geometry, more specifically in terms of its associated fan in the sense of Kato.
This formula yields a much smaller set of candidate poles for the motivic zeta function and seems especially well suited to tackle the monodromy conjecture of Halle and Nicaise for Calabi-Yau $K$-varieties, for which log smooth models appear naturally through the Gross-Siebert programme on mirror symmetry.
We end the chapter by showing how this formula sheds new light on previous results regarding the motivic zeta function of a polynomial nondegenerate with respect to its Newton polyhedron, and of a polynomial in two variables.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/abstractnl/Makefile <==
# Autogenerated Makefile, Wed Dec  3 15:26:41 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: abstractnl.pdf
abstractnl.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstractnl/$@ )

.PHONY: bare abstractnl_bare.pdf
bare: abstractnl_bare.pdf
abstractnl_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstractnl/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/abstractnl/abstractnl.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard abstractnl*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) abstractnl.pdf abstractnl_bare.pdf

s:
	@echo gvim abstractnl.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/abstractnl/abstractnl.tex <==
\chapter{Beknopte samenvatting}


In deze thesis passen we logaritmische methoden toe om motivische objecten te bestuderen.
Zij $R$ een complete discrete valuatiering met breukenveld~$K$ en perfecte residuveld~$k$.
In hoofdstuk~\ref{ch:serre} geven we een nieuwe constructie van de motivische Serre invariant van een gladde $K$-variëteit en breiden we hem additief uit tot willekeurige $K$-variëteiten.
Het voornaamste voordeel van deze constructie is dat ze enkel van resolutie van singulariteiten afhangt en niet beperkt wordt tot karakteristiek nul, in tegenstelling tot eerdere resultaten.
We geven als toepassing een voorwaardelijk positief antwoord op de vraag van Serre over het bestaan van rationale vaste punten van een $G$-actie op de affiene ruimte, waarbij $G$ een eindige $\ell$-groep is.
We sluiten dit hoofdstuk af met een andere toepassing van ons logaritmische standpunt en tonen hoe de motivische nearby cycles met drager van Guibert, Loeser en Merle beschouwd kunnen worden als een motivische volume.

%In this thesis, we use logarithmic methods to study motivic objects.
%Let $R$ be a complete discrete valuation ring with perfect residue field~$k$, and denote by $K$ its fraction field.
%We give in chapter~\ref{ch:serre} a new construction of the motivic Serre invariant of a smooth $K$-variety and extend it additively to arbitrary $K$-varieties.
%The main advantage of this construction is to rely only on resolution of singularities and not on a characteristic zero assumption, as did previous results.
%As an application, we give a conditional positive answer to Serre's question on the existence of rational fixed points of a $G$-action on the affine space, for $G$ a finite $\ell$-group.
%We end the chapter by showing how the logarithmic point of view that we use in our construction leads to a new understanding of the motivic nearby cycles with support of Guibert, Loeser and Merle as a motivic volume.

In hoofdstuk~\ref{ch:log} maken we gebruik van de theorie van logaritmische meetkunde om een nieuwe formule af te leiden voor de motivische zeta functie via de volume Poincaré reeks.
We tonen met name hoe de volume Poincaré reeks berekend kan worden vanuit een generiek gladde log-gladde $R$-schema in termen van logaritmische gegevens, in het bijzonder in termen van zijn geassocieerde waaier, in de zin van Kato.
Deze formule levert een veel kleinere verzameling van kandidaten polen op voor de motivische zeta functie, en lijkt bijzonder goed geschikt om de monodromie conjectuur van Halle en Nicaise voor Calabi-Yau variëteiten aan te pakken, waarvoor log-gladde modellen geconstrueerd kunnen worden in het kader van de Gross-Siebert programma over spiegelsymmetrie.
Ten slotte wordt er getoond aan het einde van dit hoofdstuk hoe onze formule licht werpt op eerdere resultaten omtrent de motivische zeta functie van een veelterm die niet gedegenereerd is ten opzichte van zijn Newton polyhedron, en van een veelterm in twee veranderlijken.
%In chapter~\ref{ch:log} we use the theory of logarithmic geometry to derive a new formula for the motivic zeta function via the volume Poincaré series.
%More precisely, we show how to compute the volume Poincaré series associated to a generically smooth log smooth $R$-scheme in terms of its log geometry, more specifically in terms of its associated fan in the sense of Kato.
%This formula yields a much smaller set of candidate poles for the motivic zeta function and seems especially well suited to tackle the monodromy conjecture of Halle and Nicaise for Calabi-Yau $K$-varieties, for which log smooth models appear naturally through the Gross-Siebert programme on mirror symmetry.
%We end the chapter by showing how this formula sheds new light on previous results regarding the motivic zeta function of a polynomial nondegenerate with respect to its Newton polyhedron, and of a polynomial in two variables.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/conclusion/Makefile <==
# Autogenerated Makefile, Wed Dec  3 15:26:39 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: conclusion.pdf
conclusion.pdf: 
	( cd "$(MAINDIR)" && make chapters/conclusion/$@ )

.PHONY: bare conclusion_bare.pdf
bare: conclusion_bare.pdf
conclusion_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/conclusion/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/conclusion/conclusion.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard conclusion*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) conclusion.pdf conclusion_bare.pdf

s:
	@echo gvim conclusion.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/conclusion/conclusion.tex <==
\chapter{This is conclusion}\label{ch:conclusion}

\ldots

\instructionsconclusions


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/curriculum/Makefile <==
# Autogenerated Makefile, Wed Dec  3 15:26:40 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: curriculum.pdf
curriculum.pdf: 
	( cd "$(MAINDIR)" && make chapters/curriculum/$@ )

.PHONY: bare curriculum_bare.pdf
bare: curriculum_bare.pdf
curriculum_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/curriculum/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/curriculum/curriculum.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard curriculum*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) curriculum.pdf curriculum_bare.pdf

s:
	@echo gvim curriculum.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/curriculum/curriculum.tex <==
\chapter{This is curriculum}\label{ch:curriculum}

\ldots

\instructionscv


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/formRig/Makefile <==
# Autogenerated Makefile, Fri Jan 30 13:00:49 CET 2015.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: formRig.pdf
formRig.pdf: 
	( cd "$(MAINDIR)" && make chapters/formRig/$@ )

.PHONY: bare formRig_bare.pdf
bare: formRig_bare.pdf
formRig_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/formRig/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/formRig/formRig.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard formRig*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) formRig.pdf formRig_bare.pdf

s:
	@echo gvim formRig.tex biblio.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/introduction/Makefile <==
# Autogenerated Makefile, Wed Dec  3 15:26:40 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: introduction.pdf
introduction.pdf: 
	( cd "$(MAINDIR)" && make chapters/introduction/$@ )

.PHONY: bare introduction_bare.pdf
bare: introduction_bare.pdf
introduction_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/introduction/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/introduction/introduction.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard introduction*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) introduction.pdf introduction_bare.pdf

s:
	@echo gvim introduction.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/log/Makefile <==
# Autogenerated Makefile, Wed Dec  3 15:26:40 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: log.pdf
log.pdf: 
	( cd "$(MAINDIR)" && make chapters/log/$@ )

.PHONY: bare log_bare.pdf
bare: log_bare.pdf
log_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/log/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/log/log.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard log*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) log.pdf log_bare.pdf

s:
	@echo gvim log.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/manual/Makefile <==
# Autogenerated Makefile, Wed Dec  3 15:26:40 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: manual.pdf
manual.pdf: 
	( cd "$(MAINDIR)" && make chapters/manual/$@ )

.PHONY: bare manual_bare.pdf
bare: manual_bare.pdf
manual_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/manual/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/manual/manual.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard manual*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) manual.pdf manual_bare.pdf

s:
	@echo gvim manual.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/manual/manual.tex <==
\chapter{Manual}\label{ch:manual}


\ldots

\section{Tips and Tricks}


\subsection{Full cover page}

\textbf{Important}: most printing services will create their own cover page based
on the details you send them (title, name, affiliation, ...) and do not supply
you with all necessary parameters (e.g., thickness of the paper) because these
differ from machine to machine. Therefore, the generated cover page is only
indicative and probably not used by your printing server (or even correct).


A full cover page (combining front cover, spine and back cover) can be
generated automatically using the command \texttt{make cover} or \texttt{python3 run.py cover}. This creates a pdf
\texttt{\$(COVERPDF);} by default this is \texttt{cover.pdf}.

The width of the spine is set by redefining \texttt{\\adsphdspinewidth} (9mm by default).

It can be seen in the provided \texttt{thesis.tex} that all information necessary to
generate a cover page is contained between two markers

\begin{verbatim}
    %%% COVER: Settings %%%
    ...
    %%% COVER: End settings %%%
\end{verbatim}

DO NOT REMOVE THESE!! They are used by the Makefile!!

The default front and/or back cover page can be overwritten: 

\begin{itemize}
    \item create a file \texttt{mycoverpage.tex}
    \item redefine the commands \texttt{\\makefrontcovergeneral} and \texttt{\\makebackcovergeneral}. For
          an example and more information, see the provided file \texttt{mycoverpage.tex}.
\end{itemize}

The cover page in the generated pdf has the following structure:

{\tiny
\begin{verbatim}
    <--rbleed--><--backcoverpage--><--lbleed--><--spine width--><--lbleed--><--frontcoverpage--><--rbleed-->
\end{verbatim}
}

The default bleed (both lbleed and rbleed) is 7mm. I suggest not changing this
value unless you know what you are doing ;) The latter can be done by
redefining \texttt{\\defaultlbleed} and \texttt{\\defaultrbleed} respectively.


\subsection{Finetuning the backref package}

Finetuning the backref package (when \textbf{not} using biblatex). Add the
following to your preamble:

\begin{verbatim}
% See [http://n2.nabble.com/backref-td478438.html]:
% simple backref command redefinition to avoid double entries
\makeatletter
\ifadsphd@biblatex\else
  \ifadsphd@pagebackref%
    \renewcommand*{\backref}[1]{}
    % redefinition of the actually used \backrefalt 
    \renewcommand*{\backrefalt}[4]{% 
    \ifcase #1 % 
       % case: not cited 
    \or 
       % case: cited on exactly one page 
       Cited on page~#2.
    \else 
       % case: cited on multiple pages 
       Cited on pages~#2.
    \fi}
  \else
    \renewcommand*{\backref}[1]{}
    % redefinition of the actually used \backrefalt 
    \renewcommand*{\backrefalt}[4]{% 
    \ifcase #1 % 
       % case: not cited 
    \or 
       % case: cited on exactly one page 
       Cited in Section~#2.
    \else 
       % case: cited on multiple pages 
       Cited in Sections~#2.
    \fi}
  \fi
\fi
\makeatother
\end{verbatim}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage



==> chapters/preface/Makefile <==
# Autogenerated Makefile, Wed Dec  3 15:26:40 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: preface.pdf
preface.pdf: 
	( cd "$(MAINDIR)" && make chapters/preface/$@ )

.PHONY: bare preface_bare.pdf
bare: preface_bare.pdf
preface_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/preface/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/preface/preface.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard preface*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) preface.pdf preface_bare.pdf

s:
	@echo gvim preface.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/preface/preface.tex <==
\chapter{Dankwoord} \label{ch:preface}


Het einde van deze doctoraat hoort samen met het einde van mijn Leuvense avontuur.
De eerste mensen die ik graag wil bedanken zijn allen die ervoor hebben gezorgd dat ik me welkom en helemaal op mijn plaats voelde in Leuven.
Het begon al bijna 6 jaar geleden toen ik contact met Johan Quaegebeur opnam om meer informatie te krijgen over het volgen van bepaalde mastervakken in KU~Leuven.
Zijn vriendelijke antwoord was voor mij het eerste teken dat Leuven zo'n gastvrije plaats was.
Dat jaar heb ik de toenmalige groep master-1-studenten leren kennen en mijn goede ervaringen bij hen hebben me aangespoord om door te zetten: het jaar erop maakte ik kennis met Johannes en begon ik Hartshorne te studeren onder de begeleiding van Lorenzo in het research vak algebraïsche meetkunde.
Op het einde van het semester had ik besloten aan een doctoraat te beginnen in dat vak, en mocht ik horen van Johannes dat er plaats voor mij in Leuven was.
Een paar maanden later kwam goed nieuws uit het FWO; ik wil het hier graag bedanken voor het mandaat dat ik kreeg toegekend en zonder welke alles een stuk ingewikkelder zou verlopen zijn.

Mijn jaren als doctoraatstudent zouden heel anders zijn geweest was ik niet omringd door buitengewone collega's, die voor zo'n goede sfeer zorgden. Ze hebben allemaal op hun eigen manier bijgedragen tot de kwaliteit van mijn verblijf in Leuven.
%Mopjes van studenten ga ik ook missen.

The last mathematicians I would like to thank are the members of my examination commitee, who accepted to go through this work for the final phase of my PhD: many thanks to Nero Budur, Arno Kuijlaars, Michel Raibaut, Julien Sebag, Wim Veys and, of course, my adviser Johannes Nicaise, whose constant support and insights have got me back on track more than once.%who was very supportive.

Het leven in Leuven was ook rijk aan ontmoetingen buiten de universiteit, wat voor goed evenwicht zorgde tussen wiskunde en werkelijkheid.
In het bijzonder wil ik graag bedanken: mijn huisgenoot Wim voor de talrijke zwem- en joggingsessies en zijn \emph{regard décalé sur la vie}, mijn partijgenoot David voor de talloze inspirerende gesprekken, en mijn pianoleerkracht Hester, die mij in een nieuwe wereld heeft begeleid.

Famille et amis ont également grandement contribué à l'achèvement de ce travail par leur présence et leur soutien moral. Je tiens à remercier en particulier Valérian, avec qui j'ai pu partager les vicissitudes du métier de chercheur, mes parents, pour leur soutien indéfectible et leur enthousiasme sans borne et surtout Maëlle, pour sa patience, ses encouragements et pour avoir toujours su être là quand il le fallait. Et, oui, la Gaume c'est joli.

Je terminerai par une pensée pour ma grand-mère, qui n'aura pas eu le plaisir de voir mon travail achevé, mais qui, je n'en doute pas, en aurait été immensément fière.


\vspace{2em}

\hfill\begin{minipage}[t]{.15\textwidth}
\raggedright{\emph{À Bon-papa}}
\end{minipage}




%De eerste mensen dat ik graag wil bedanken is de bende die ervoor hebben gezorgd dat er zo'n goede sfeer hing: Bart & Bart, Berdien, Clara, David, Jan, Jonas, Niels, Thomas. Ook Arno Kuijlaars wil ik hier bedan


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/prelim_log/Makefile <==
# Autogenerated Makefile, Thu Dec  4 15:56:59 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: prelim_log.pdf
prelim_log.pdf: 
	( cd "$(MAINDIR)" && make chapters/prelim_log/$@ )

.PHONY: bare prelim_log_bare.pdf
bare: prelim_log_bare.pdf
prelim_log_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/prelim_log/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/prelim_log/prelim_log.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard prelim_log*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) prelim_log.pdf prelim_log_bare.pdf

s:
	@echo gvim prelim_log.tex defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/serre/Makefile <==
# Autogenerated Makefile, Wed Dec  3 15:26:46 CET 2014.

MAINDIR = /home/manu/math/thèse KUL/manuscrit/adsphd-master

.PHONY: serre.pdf
serre.pdf: 
	( cd "$(MAINDIR)" && make chapters/serre/$@ )

.PHONY: bare serre_bare.pdf
bare: serre_bare.pdf
serre_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/serre/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/manu/math/thèse KUL/manuscrit/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/serre/serre.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard serre*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) serre.pdf serre_bare.pdf

s:
	@echo gvim serre.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

\makeatother

